Frequency-explicit a posteriori error estimates for discontinuous Galerkin discretizations of Maxwell's equations

We propose a new residual-based a posteriori error estimator for discontinuous Galerkin discretizations of time-harmonic Maxwell's equations in first-order form. We establish that the estimator is reliable and efficient, and the dependency of the reliability and efficiency constants on the frequency is analyzed and discussed. The proposed estimates generalize similar results previously obtained for the Helmholtz equation and conforming finite element discretization of Maxwell's equations. In addition, for the discontinuous Galerkin scheme considered here, we also show that the proposed estimator is asymptotically constant-free for smooth solutions. We also present two-dimensional numerical examples that highlight our key theoretical findings and suggest that the proposed estimator is suited to drive $h$- and $hp$-adaptive iterative refinements.

==> approximation_factor.tex <==
We consider the case where
$\ee = \eps \BTI_3$ and $\mm = \mu \BTI_3$
for two real strictly positive constants $\eps,\mu \in \mathbb R$,
and $\Omega$ is of class $\CC^{k+1,1}$. %% TODO: check
For the sake of shortness, we only consider the ``electric''
problem here, but the ``magnetic'' problem can be dealt \pvr{by}
following the same procedure. In particular, notice that
the shift-regularity results of Section \ref{sec_shift_curl} below
work for both types of boundary conditions.

\subsection{High-order Sobolev spaces}

In addition to the first-order Sobolev spaces introduced at Section
\ref{functional_spaces}\pvr{, w}e will need, for $m \geq 0$, the high-order
Sobolev space $\BCH^m(\Omega)$ of functions $\bv \in \BLL^2(\Omega)$ such
that $\partial^{|\alpha|} \bv/\partial^\alpha \bx \in \BLL^2(\Omega)$ for all $|\alpha| \leq m$,
see e.g. \cite{adams_fournier_2003a}. This space is equipped with the norm
\begin{equation*}
\|\bv\|_{\BCH^m}^2
\eq
\sum_{j=0}^m
\left (
\ell_\Omega^j \sum_{|\alpha| = j}
\left \|\frac{\partial^{|\alpha|} \bv}{\partial^\alpha \bx}\right \|_\Omega^2
\right ).
\end{equation*}

\subsection{High-order interpolation}

Following \cite{ern_guermond_2017a}, and assuming that $0 \leq m \leq k$, we have
\begin{equation*}
\|\bw - \CR_h \bw\|_\Omega \leq \cI h^{m+1} \|\bw\|_{\BCH^{m+1}},
\qquad
\|\curl(\bw - \CR_h \bw)\|_\Omega \leq \cI h^{m+1} \|\curl \bw\|_{\BCH^{m+1}}
\end{equation*}
for all $\bw \in \BCH_0(\ccurl,\Omega) \cap \BCH^{m+1}(\Omega)$,
where the constant $\cI$ only depends on $k$ and the shape-regularity
parameter $\beta$.

\subsection{Regularity pick-up}
\label{sec_shift_curl}

Let $\bv \in \BCH(\ccurl,\Omega) \cap \BCH(\ddiv^0,\Omega)$,
with either $\bv \times \bn = \bo$ or $\bv \cdot \bn = o$ on $\partial \Omega$.
Then, for all $0 \leq m \leq k$, if $\curl \bv \in \BCH^m(\Omega)$,
then we have $\bv \in \BCH^{m+1}(\Omega)$ with
\begin{equation}
\label{eq_curl_shift}
\|\bv\|_{\BCH^{m+1}} \leq \cD \ell_\Omega \|\curl \bv\|_{\BCH^m},
\end{equation}
where the constant $\cD$ only depends on $\Omega$ and $k$.
We refer the reader to Corollary 3.7 of \cite{girault_raviart_1986a}.
Notice in particular that if $m \leq k-1$ and
$\bu \in \BCH_0(\ccurl,\omega) \cap \BCH(\ddiv^0,\Omega)$
satisfies $\curl \curl \bu \in \BCH^m$, then
\begin{equation}
\label{eq_curl_double_shift}
\|\bu\|_{\BCH^{m+2}}
\leq
\cD^2 \ell_\Omega^2 \|\curl \curl \bu\|_{\BCH^m}.
\end{equation}

%% TODO: we only have a reference for magnetic boundary conditions,
%% we are missing electric boundary conditions.

\subsection{Rescaling}

Let $\bj \in \BCH(\ddiv^0,\Omega)$. Introducing
$K \eq \omega \ell_\Omega/c$ and $\bg \eq (\ell_\Omega/c) \bj$,
we may rewrite equation \eqref{eq_def_be_bj} defining $\be \eq \be^\star(\bj)$ as
% \begin{equation*}
% -\omega^2 \eps \be + \chi \curl \curl \be = \eps \omega \bj,
% \end{equation*}
% and we note that $\be \in \BCH(\ddiv^0,\Omega)$. Then, multiplying by $\mu \ell_\Omega^2$,
% we obtain that
\begin{equation}
\label{eq_maxwell_scaled}
-K^2 \be + \ell_\Omega^2 \curl \curl \be = K \bg.
\end{equation}
In addition, it follows from \eqref{eq_cS} that
\begin{equation}
\label{eq_stab_rescaled}
K^2 \|\be\|_\Omega^2 + \ell_\Omega^2 \|\curl \be\|_\Omega^2
\leq
\cSE^2 \|\bg\|_\Omega^2.
\end{equation}

\subsection{Stability}

The problem under consideration is self-adjoint, as we consider
real-valued coefficients $\ee$ and $\mm$. We may thus introduce
a sequence of eigenpairs $\{(\lambda_j,\bphi_j)\}_{j \geq 0}$
such that $\ell_\Omega^2 \curl \curl \bphi_j = \lambda_j \bphi_j$.
Classically, we chose the normalization $\|\bphi_j\|_{\Omega} = 1$,
so that $\{\bphi_j\}_{j \geq 0}$ and $\{\sqrt{\lambda_j} \bphi_j\}_{j \geq 0}$
are orthonormal basis of $\BCH(\ddiv^0,\Omega)$ and
$\BCH_0(\ccurl,\Omega) \cap \BCH(\ddiv^0,\Omega)$, respectively.
We also introduce $D \eq \min_{j \geq 0} |\sqrt{\lambda_j} - K|$, and
$\delta \eq \min_{j \geq 0}|\omega_j - \omega|$, with
$\omega_j \eq c \sqrt{\lambda_j}/\ell_\Omega$.

\begin{theorem}[Stability]
The estimates
\begin{equation}
\label{eq_stability_estimates}
K \|\be\|_\Omega \leq \frac{K}{D} \|\bg\|_\Omega,
\qquad
\ell_\Omega \|\curl \be\|_\Omega \leq \frac{K}{D} \|\bg\|_\Omega
\end{equation}
and
\begin{equation}
\label{eq_estimate_cSE}
\cSE \leq \frac{\omega}{\delta},
\end{equation}
hold true.
\end{theorem}

\begin{proof}
Since $\be,\bg \in \BCH(\ddiv^0,\Omega)$, we may expand $\be$ and $\bg$
in the basis $\{\bphi_j\}_{j \geq 0}$ by letting $e_j \eq (\be,\bphi_j)$
and $g_j \eq (\be,\bphi_j)$. Then, we see from \eqref{eq_maxwell_scaled} that
\begin{equation*}
|e_j|
=
\frac{K}{|\lambda_j-K^2|} |g_j|
\leq
\frac{1}{D}\frac{K}{\sqrt{\lambda_j}+K} |g_j|\quad
\text{ and }
\quad\left (K + \sqrt{\lambda_j}\right )|e_j|
\leq
\frac{K}{D} |g_j|.
\end{equation*}
Then, \eqref{eq_stability_estimates} follows from
\begin{equation*}
K^2\|\be\|_\Omega^2 + \ell_\Omega^2 \|\curl \be\|_\Omega^2
=
\sum_{j \geq 0}
(K^2 + \lambda_j)|e_j|^2
\leq
\sum_{j \geq 0}
\left ( (K + \sqrt{\lambda_j})|e_j|\right )^2
\leq
\left (\frac{K}{D}\right )^2 \|\bg\|_\Omega^2.
\end{equation*}
Estimate \eqref{eq_estimate_cSE} follows by multiplying the above estimate by $\chi/\ell_\Omega^2$.
\end{proof}

\subsection{Basic regularity}

We first establish a basic regularity result for $\be$.
Notice that while this result would be sufficient to derive
sharp estimates when $k=0$, additional work is required for
high-order methods.

\begin{lemma}[Basic regularity]
\label{lemma_basic_regularity}
We have
\begin{equation}
\label{eq_basic_reg_be}
K \|\be\|_{\BCH^1} \leq \cD \cSE K \|\bg\|_{\BCH^0},
\end{equation}
and
\begin{equation}
\label{eq_basic_reg_curl_be}
\ell_\Omega \|\curl \be\|_{\BCH^1} \leq \cD (1+\cSE) K \|\bg\|_{\BCH^0}.
\end{equation}
\end{lemma}

\begin{proof}
Shift estimate \eqref{eq_curl_shift} and stability estimate \eqref{eq_stab_rescaled} imply that
\begin{equation*}
\|\be\|_{\BCH^1}
\leq
\cD \ell_\Omega \|\curl \be\|_{\BCH^0}
\leq
\cD \cSE \|\bg\|_{\BCH^0},
\end{equation*}
and \eqref{eq_basic_reg_be} follows.
On the other hand, we establish \eqref{eq_basic_reg_curl_be} by
\begin{multline*}
\ell_\Omega \|\curl \be\|_{\BCH^1}
\leq
\cD \ell_\Omega^2 \|\curl \curl \be\|_{\BCH^0}
\\
\leq
\cD \left (K \|\bg\|_{\BCH^0} + K^2 \|\be\|_{\BCH^0}\right )
\leq
\cD (1+\cSE) K\|\bg\|_{\BCH^0}.
\end{multline*}
\end{proof}

\subsection{Expansion}

As we only have a limited regularity assumption for the right-hand side $\bg$,
we may not expect more regularity than established in Lemma \ref{lemma_basic_regularity}
for the associated solution $\be$. As shown in
\cite{chaumontfrelet_nicaise_2019a,melenk_sauter_2011a} for the Helmholtz equation,
the key idea is to introduce a ``regularity splitting'' of the solution. Here, we
shall adapt the approach of \cite{chaumontfrelet_nicaise_2019a} to Maxwell's equations,
and consider the formal expansion
\begin{equation}
\label{eq_formal_expansion}
\be = \sum_{j \geq 0} K^j \be_j.
\end{equation}
After identifying the powers in \eqref{eq_maxwell_scaled}, one sees that
$\be_0 \eq \bo$, and that the other elements
$\be_j \in \BCH_0(\ccurl,\Omega) \cap \BCH(\ddiv^0,\Omega)$
are iteratively defined through
%\begin{subequations}
\begin{equation}
%\label{eq_def_be1}
\label{eq_def_be}
\ell_\Omega^2 \curl \curl \be_1 = \bg,
\qquad
\text{and}\qquad\ell_\Omega^2 \curl \curl \be_j = \be_{j-2}
\end{equation}
for $j \geq 2$. We first show that the iterates in the sequence exhibit
increasing regularity.

\begin{lemma}[Increasing regularity of the expansion]
For all $j \geq 0$, we have $\be_j \in \BCH^{j+1}(\Omega)$
and $\curl \be_j \in \BCH^j(\Omega)$ with
\begin{equation}
\label{eq_bej}
\|\be_j\|_{\BCH^{j+1}}
\leq
\cD^{j+1} \|\bg\|_{\BCH^0},
\end{equation}
and
\begin{equation}
\label{eq_curl_bej}
\ell_\Omega \|\curl \be_j\|_{\BCH^j}
\leq
\cD^j \|\bg\|_{\BCH^0}.
\end{equation}
\end{lemma}

\begin{proof}
We start with \eqref{eq_curl_bej}. It obviously holds for $j = 0$
as $\be_0 \eq \bo$. For $j=1$, recalling  %\eqref{eq_def_be1}
\eqref{eq_def_be}, we have
\begin{equation*}
\ell_\Omega \|\curl \be_1\|_{\BCH^1}
\leq
\cD \ell_\Omega^2 \|\curl \curl \be_1\|_{\BCH^0}
\leq
\cD \|\bg\|_{\BCH^0}.
\end{equation*}
Then, assuming that \eqref{eq_curl_bej} holds up to some $j$, \eqref{eq_curl_shift} and \eqref{eq_def_be} 
reveal that
\begin{multline*}
\ell_\Omega \|\curl \be_{j+2}\|_{\BCH^{j+2}}
\leq
\cD \ell_\Omega^2 \|\curl \curl \be_{j+2}\|_{\BCH^{j+1}}
\leq
\cD^2 \ell_\Omega \|\curl \be_j\|_{\BCH^j}
\leq
\cD^{j+2} \|\bg\|_{\BCH^0},
\end{multline*}
and \eqref{eq_curl_bej} follows by induction.

On the other hand, \eqref{eq_bej} is a direct consequence
of \eqref{eq_curl_bej}, since \eqref{eq_curl_shift} shows that
\begin{equation*}
\|\be_j\|_{\BCH^{j+1}}
\leq
\cD \ell_\Omega \|\curl \be_j\|_{\BCH^j}
\leq
\cD \left (\cD^j \|\bg\|_{\BCH^0}\right ).
\end{equation*}
\end{proof}

So far, expansion \eqref{eq_formal_expansion} is only formal, and we need to
cut the expansion into a finite sum. To do so, we introduce,
for $\ell \geq 0$, the ``residual'' term
\begin{equation*}
\br_\ell \eq \be - \sum_{j=0}^\ell \omega^j \be_j
\in
\BCH_0(\ccurl,\Omega) \cap \BCH(\ddiv^0,\Omega),
\end{equation*}
so that $\be
=
\sum_{j=0}^\ell K^j \be_j
+
\br_\ell$.

As we show next, these residuals have increasing regularity.

\begin{lemma}[Regularity of residual terms]
We have
\begin{equation}
\label{eq_br}
K\|\br_\ell\|_{\BCH^{\ell+1}} \leq \cSE (\cD K)^{\ell+1} \|\bg\|_{\BCH^0},
\end{equation}
and
\begin{equation}
\label{eq_curl_br}
\ell_\Omega \|\curl \br_\ell\|_{\BCH^{\ell+1}} \leq (1+\cSE) (\cD K)^{\ell+1} \|\bg\|_{\BCH^0}.
\end{equation}
\end{lemma}

\begin{proof}
We have $\br_0 \eq \be$, so that \eqref{eq_br} and \eqref{eq_curl_br} holds for $\ell=0$
as a direct consequence of \eqref{eq_basic_reg_be} and \eqref{eq_basic_reg_curl_be}.

For the case $\ell=1$, simple computations show that
$\ell_\Omega^2 \curl \curl \br_1 = K^2 \be$.
It then follows from \eqref{eq_basic_reg_be} that
\begin{align*}
K \|\br_1\|_{\BCH^2}
\leq
K \cD^2 \ell_\Omega^2 \|\curl \curl \br_1\|_{\BCH^0}
\leq
\cD^2 K^3\|\be\|_{\BCH^0}
\leq
\cSE \cD^2 K^2 \|\bg\|_{\BCH^0},
\end{align*}
and
\begin{equation*}
\ell_\Omega \|\curl \br_1\|_{\BCH^2}
\leq
\cD
\ell_\Omega^2 \|\curl \curl \br_1\|_{\BCH^1}
\leq
\cD K^2 \|\be\|_{\BCH^1}
\leq
\cSE \cD^2 K^2 \|\bg\|_{\BCH^0},
\end{equation*}
so that \eqref{eq_br} and \eqref{eq_curl_br} are also valid when $\ell=1$.

For the general case, we first observe that
$\ell_\Omega^2 \curl \curl \br_{\ell+2} = K^2 \br_\ell$.
Therefore, using \eqref{eq_curl_shift} and \eqref{eq_curl_double_shift}, we have
\begin{equation*}
\|\br_{\ell+2}\|_{\BCH^{\ell+3}}
\leq
\cD^2 K^2 \|\br_\ell\|_{\BCH^{\ell+1}},
\end{equation*}
and
\begin{multline*}
\ell_\Omega \|\curl \br_{\ell+2}\|_{\BCH^{\ell+3}}
\leq
\cD \ell_\Omega^2
\|\curl \curl \br_{\ell+2}\|_{\BCH^{\ell+2}}
\\
\leq
\cD K^2
\|\br_{\ell}\|_{\BCH^{\ell+2}}
\leq
\cD^2 K^2 \ell_\Omega \|\curl \br_\ell\|_{\BCH^{\ell+1}},
\end{multline*}
and the general case follows by induction.
\end{proof}

\subsection{Approximation factor}

We are now ready to provide an upper bound for the approximation factor $\gbaE$.

\begin{theorem}[Approximation factor]
Assume that $\cD (\omega h/c) \leq 1/2$, then the following estimate holds true
\begin{equation*}
% \label{eq_estimate_gba}
\gbaE
\leq
\cI
\left (
2 \sqrt{2} \cD \frac{\omega h}{c}
+
\sqrt{1+2\cSE^2}
\left (\cD\frac{\omega h}{c}\right )^{k+1}
\right ).
\end{equation*}
\end{theorem}

\begin{proof}
Let be $ \ell\geq 1 $ and $ j=1,\ldots,\ell $. Recalling \eqref{eq_gba_second_order}
and the finite expansion for $ \be $, it is sufficient to provite upper bounds for the high
order interpolation error of $ \be_j $ and $ \br_{\ell} $. For $ \be_j $, the definition
of $K$ and \eqref{eq_def_be} imply that
\begin{equation*}
K^{j+1}\|\be_j-\CR_h \be_j\|_{\BCH^0}
\leq
\cI
K^{j+1} \frac{h^{j+1}}{\ell_\Omega^{j+1}} \|\be_j\|_{\BCH^{j+1}}
=
\cI
\left (\frac{\omega h}{c}\right )^{j+1} \|\be_j\|_{\BCH^{j+1}}
\leq
\cI
\left (\cD \frac{\omega h}{c}\right )^{j+1} \|\bg\|_{\BCH^0},
\end{equation*}
and
\begin{equation*}
\ell_\Omega K^j \|\curl (\be_j-\CR_h \be_j)\|_{\BCH^0}
\leq
\cI
K^j \frac{h^j}{\ell_\Omega^j} \ell_\Omega \|\curl \be_j\|_{\BCH^{j}}
\leq
\cI
\left ( \cD \frac{\omega h}{c} \right )^j \|\bg\|_{\BCH^0},
\end{equation*}
and since $\cD (\omega h/c) \leq 1$, we get
\begin{equation*}
K^j \left (
K^2\|\be_j-\CR_h \be_j\|_{\BCH^0}^2
+
\ell_\Omega^2 \|\curl (\be_j-\CR_h \be_j)\|_{\BCH^0}^2
\right )^{1/2}
\leq
\cI
\sqrt{2} \left ( \cD \frac{\omega h}{c} \right )^j \|\bg\|_{\BCH^0}.
\end{equation*}

Similarly, for the residual $ \br_{\ell} $, we have
\begin{align*}
K \|\br_k-\CR_h \br_k\|_{\BCH^0}
\leq
\cI \left ( \frac{h}{\ell_\Omega} \right )^{k+1} K\|\br_k\|_{\BCH^{k+1}}
\leq
\cI \cSE \left (\cD \frac{\omega h}{c} \right )^{k+1} \|\bg\|_{\BCH^0}
\end{align*}
and
\begin{align*}
\ell_\Omega \|\curl (\br_k-\CR_h \br_k)\|_{\BCH^0}
\leq
\cI
\left (\frac{h}{\ell_\Omega}\right )^{k+1}
\ell_\Omega \|\curl \br_k\|_{\BCH^{k+1}}
\leq
\cI
(1+\cSE)
\left ( \cD \frac{\omega h}{c} \right )^{k+1}
\|\bg\|_{\BCH^0},
\end{align*}
and hence
\begin{equation*}
K^2 \|\br_k - \CR_h \br_k\|_{\BCH^0}^2
+
\ell_\Omega^2 \|\curl (\br_k - \CR_h \br_k)\|_{\BCH^0}^2
\leq
\cI \sqrt{1+2\cSE^2} \left ( \cD \frac{\omega h}{c} \right )^{k+1} \|\bg\|_{\BCH^0}.
\end{equation*}

Then, since $\be = \sum_{j=1}^k K^j \be_j + \br_k$ and the above estimates, we obtain
\begin{multline*}
K^2 \|\be - \CR_h \be\|_{\BCH^0}^2
+
\ell_\Omega^2 \|\curl (\be - \CR_h \be)\|_{\BCH^0}^2
\\
\leq
\cI \left (
\sqrt{2}
\sum_{j=1}^k \left (\cD \frac{\omega h}{c}\right )^j
+
\sqrt{1+2\cSE^2} \left ( \cD \frac{\omega h}{c} \right )^{k+1}
\right )
\|\bg\|_{\BCH^0}.
\end{multline*}
Finally, the result follows by
\begin{align*}
\sum_{j=1}^k \left (\cD \frac{\omega h}{c}\right )^j
=
\left (\cD \frac{\omega h}{c}\right )\sum_{j=0}^{k-1} \left (\cD \frac{\omega h}{c}\right )^j
&=
\left (\cD \frac{\omega h}{c}\right )
\frac{1 - \left (\cD \frac{\omega h}{c}\right )^{k}}{1 - \left (\cD \frac{\omega h}{c}\right )}
\leq
2\cD \frac{\omega h}{c}.
\end{align*}
\end{proof}

\begin{corollary}[Simplified estimate]
Assume that $\cD (\omega h/c) \leq 1/2$ and $\omega \geq \delta$, then
\begin{equation}
\label{eq_estimate_gbaE_simplified}
\gbaE
\leq
C(\Omega,k) \left (
\frac{\omega h}{c} + \frac{\omega}{\delta} \left (\frac{\omega h}{c}\right )^{k+1}
\right ).
\end{equation}
\end{corollary}

